This Sample seems to be good enough! Assessing Coverage and Temporal Reliability of Twitter's Academic API

Because of its willingness to share data with academia and industry, Twitter has been the primary social media platform for scientific research as well as for consulting businesses and governments in the last decade. In recent years, a series of publications have studied and criticized Twitter's APIs and Twitter has partially adapted its existing data streams. The newest Twitter API for Academic Research allows to "access Twitter's real-time and historical public data with additional features and functionality that support collecting more precise, complete, and unbiased datasets." The main new feature of this API is the possibility of accessing the full archive of all historic Tweets. In this article, we will take a closer look at the Academic API and will try to answer two questions. First, are the datasets collected with the Academic API complete? Secondly, since Twitter's Academic API delivers historic Tweets as represented on Twitter at the time of data collection, we need to understand how much data is lost over time due to Tweet and account removal from the platform. Our work shows evidence that Twitter's Academic API can indeed create (almost) complete samples of Twitter data based on a wide variety of search terms. We also provide evidence that Twitter's data endpoint v2 delivers better samples than the previously used endpoint v1.1. Furthermore, collecting Tweets with the Academic API at the time of studying a phenomenon rather than creating local archives of stored Tweets, allows for a straightforward way of following Twitter's developer agreement. Finally, we will also discuss technical artifacts and implications of the Academic API. We hope that our work can add another layer of understanding of Twitter data collections leading to more reliable studies of human behavior via social media data.

==> decay_long.tex <==
\begin{figure}[h]
\centering
\footnotesize
\begin{tikzpicture}
\begin{axis}[
	xlabel=Months,
	ylabel=Coverage,
	width=15cm,height=6cm,
	xmin=4,xmax=79,ymax=0.82,ymin=0.48,
	ytick={0.8,0.7,0.6,0.5},
	xtick={6,12,18,24,30,36,42,48,54,60,66,72,78},
    y label style={yshift=-.8em}, x label style={yshift=.5em}]
\addplot [only marks, mark size=1pt]
table[x index=0, y index=1] {
6	0.7752
7	0.7500
8	0.7543
9	0.7544
10	0.7359
11	0.7199
12	0.7168
13	0.7169
14	0.7223
15	0.7222
16	0.7060
17	0.6960
18	0.7051
19	0.6984
20	0.7142
21	0.6818
22	0.6840
23	0.6882
24	0.6675
25	0.6902
26	0.6829
27	0.6824
28	0.6763
29	0.6526
30	0.6562
31	0.6820
32	0.6782
33	0.6523
34	0.6563
35	0.6508
36	0.6519
37	0.6443
38	0.6372
43	0.6401
44	0.6208
45	0.6098
46	0.6084
47	0.5971
48	0.6211
49	0.5983
50	0.6034
51	0.6053
52	0.6015
53	0.5794
54	0.6052
55	0.5953
56	0.5899
57	0.5889
58	0.5522
59	0.5794
60	0.5835
61	0.5707
62	0.5786
63	0.5890
64	0.5745
65	0.5436
66	0.5684
67	0.5374
68	0.5752
69	0.5627
70	0.5353
71	0.5650
72	0.5561
73	0.5818
74	0.5744
75	0.5401
76	0.5581
77	0.5536
};
\addplot []
table[x index=0, y index=1] {
6	0.7569
7	0.7531
8	0.7493
9	0.7456
10	0.7419
11	0.7382
12	0.7345
13	0.7308
14	0.7271
15	0.7235
16	0.7199
17	0.7163
18	0.7127
19	0.7091
20	0.7056
21	0.7021
22	0.6986
23	0.6951
24	0.6916
25	0.6881
26	0.6847
27	0.6813
28	0.6779
29	0.6745
30	0.6711
31	0.6677
32	0.6644
33	0.6611
34	0.6578
35	0.6545
36	0.6512
37	0.6480
38	0.6447
39	0.6415
40	0.6383
41	0.6351
42	0.6319
43	0.6288
44	0.6256
45	0.6225
46	0.6194
47	0.6163
48	0.6132
49	0.6101
50	0.6071
51	0.6040
52	0.6010
53	0.5980
54	0.5950
55	0.5921
56	0.5891
57	0.5862
58	0.5832
59	0.5803
60	0.5774
61	0.5745
62	0.5716
63	0.5688
64	0.5659
65	0.5631
66	0.5603
67	0.5575
68	0.5547
69	0.5519
70	0.5492
71	0.5464
72	0.5437
73	0.5410
74	0.5383
75	0.5356
76	0.5329
77	0.5302
};
\end{axis}
\end{tikzpicture}
\caption{Coverage over time. Proportion of 10,000 Tweets that could be found on Twitter between $0.5$ and $5.5$ years after the Tweets have been created.}
\label{fig:coverage_long} 
\end{figure}

